Scalable Wavelength Arbitration for Microring-based DWDM Transceivers

This paper introduces the concept of autonomous microring arbitration, or wavelength arbitration, to address the challenge of multi-microring initialization in microring-based Dense-Wavelength-Division-Multiplexed (DWDM) transceivers. This arbitration is inherently policy-driven, defining critical system characteristics such as the spectral ordering of microrings. Furthermore, to facilitate large-scale deployment, the arbitration algorithms must operate independently of specific wavelength information and be resilient to system variability. Addressing these complexities requires a holistic approach that encompasses the entire system, from device-level variabilities to the transceiver electrical-to-optical interface - this system-wide perspective is the focus of this paper. To support efficient analysis, we develop a hierarchical framework incorporating an ideal, wavelength-aware arbitration model to examine arbitration failures at both the policy and algorithmic levels. The effectiveness of this approach is demonstrated in two ways: by analyzing the robustness of each policy in relation to device variabilities, and by developing an algorithm that achieves near-perfect alignment with the ideal model, offering superior robustness compared to the traditional sequential tuning method. The simulator code used in this paper is available at https://github.com/wdmsim/wdm-simulator.

==> include/alg_bem.tex <==

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{algorithm}
\caption{Best-Effort Matching}
\label{alg:bem}
\begin{algorithmic}[1]
%\INPUT{\ \\
%Current microring index $i$\\
%Next microring index $j$\\
%Current microring search table $ST$
%}
\INPUT{Target spectral ordering $\{s_{i}\}$, search table $ST$ and relation index list $\{r_{ij}\}$}
\OUTPUT{Selected lock target list \{$t_{i}$\}}


\State{Construct a list of index pairs $\{ij\}$ by consecutive pairing in $\{s_{i}\}$ including the last with the first element}
\State{Initialize empty lock allocation table $LAT$}
\State{Initialize empty lock target list $t_{i}$}

\For{$i, j \gets \{ij\}$}
	\If{$r_{ij} = \text{null}$}
		\State{$NullCount \gets NullCount + 1$}
	\EndIf
	%\State{Find the relation index $r_{ij}$ in $\{r_{ij}\}
\EndFor

\If{$NullCount = 0$}\Comment{Fig.X (a) \[1\]}
	\State{$LAT \gets$ \textproc{AssemLAT}({$\{ij\}, \{r_{ij}\}, ST$}})
	%\State{Find diagonal in $LAT$ and corresponding $t_{i}$ in $ST$}
	\State{Find diagonal in $LAT$}
	\State{Find corresponding $t_{i}$ in $ST$}
\ElsIf{$NullCount = 1$}\Comment{Fig.X (b)}
	%\State{Shift $\{ij\}, r_{ij}, ST$ until $1^{st}$ idx is after $r_{ij}$ \text{null}}
	\State{Shift $\{ij\}$ until $1^{st}$ idx is after $r_{ij}$ \text{null}}
	\State{$LAT \gets$ \textproc{AssemLAT}({$\{ij\}, \{r_{ij}\}, ST$}})
	%\State{Find diagonal in $LAT$ and corresponding $t_{i}$ in $ST$}
	\State{Find diagonal in $LAT$}
	\State{Find corresponding $t_{i}$ in $ST$}
\ElsIf{$NullCount \geq 2$}\Comment{Fig.X (c)}
	%\State{Shift $\{ij\}, r_{ij}, ST$ until $1^{st}$ idx is after $r_{ij}$ \text{null}}
	\State{Shift $\{ij\}$ until $1^{st}$ idx is after $r_{ij}$ \text{null}}
	\State{Form a subgroup from $\{ij\}$ that are connected by $r_{ij}$}
	\ForEach{subgroup $\{ij\}_s$}
		\State{$SubLAT \gets$ \textproc{AssemLAT}({$\{ij\}_s, \{r_{ij}\}_s, ST_s$})}
		%\State{Find diagonal in $SubLAT$ and corresponding $t_{i}$ in $ST_s$}
		\State{Find diagonal in $LAT$}
		\State{Find corresponding $t_{i}$ in $ST$}
	\EndFor
	\State{Assemble $t_{i}$ from subgroups}
\EndIf

\State{\textbf{return} $t_{i}$}

% Add vertical space between the main function and the procedure
\vspace{1em}

\Procedure{AssemLAT}{$\{ij\}, r_{ij}, SubST$}\\
\Comment{Assemble Lock Allocation Table for the (sub)-group}
	\State{Initialize empty lock allocation table $SubLAT$}

	\State{$i \gets$ the first index of $\{ij\}$}
	\State{$SubLAT[i] \gets SubST[i]$}

	\For{$i, j \gets \{ij\}$}\Comment{Fig.X (a\-c)}
		\State{$SubLAT[j] \gets SubLAT[i] + r_{ij}$}
	\EndFor
	\State{\textbf{return} $SubLAT$}
\EndProcedure


\end{algorithmic}
\end{algorithm}





==> include/alg_rs.tex <==

\begin{algorithm}
\caption{Relation Search}
\label{alg:rs}
\begin{algorithmic}[1]
%\INPUT{\ \\
%Current microring index $i$\\
%Next microring index $j$\\
%Current microring search table $ST$
%}
\INPUT{Microring index pair $i$,$j$}
\OUTPUT{Relation index $RI_{ij}$}

%\State{Initialize $RI_{ij,cand}[2]$, $ST[vct]$ and $MaskedST[vct]$}
\State{Initialize $RI_{ij,cand}$, $ST[vct]$ and $MaskedST[vct]$}

\If{$i \leq j$}\Comment{Determine aggressor/victim}
	\State{$aggr, vct, flip \gets Ring_{i}, Ring_{j}, 1$}
\Else
	\State{$aggr, vct, flip \gets Ring_{i}, Ring_{j}, -1$}
\EndIf

%\State{/* Find the relation by microring aggression, Fig.X /*}

%%\For{$tgt \gets 0, -1$}\Comment{Fig.X (a),(b), respectively}
%\State{$aggr\_tgts \gets \{0, -1\}$
%\For{$tgt \textbf{ in } aggr\_tgts$}\Comment{Fig.X (a),(b), respectively}
%    \State{$\Call{WaveLock}{aggr, tgt}$}
%    \State{$MaskedST_{vct} \gets$ \Call{WaveSearch}{vct}}
%    \State{$RI_{ij,cand}[tgt] \gets$ SET\_DIFF$(ST[vct], MaskedST[vct])$}
%    \State{$\Call{WaveUnlock}{aggr}$}
%\EndFor

%\State{$ST_{vct} \gets \Call{WaveSearch}{vct}$}
\State{$ST[vct] \gets \Call{WaveSearch}{vct}$}
\State{$aggr\_tgts \gets \{0, -1\}$}
\State{/* $aggr\_tgts \gets \{0, -1, 1\}$ */} \Comment{Variation-Tolerant RS}
\For{$tgt \textbf{ in } aggr\_tgts$} \Comment{See Fig.11}
    \State{$\Call{WaveLock}{aggr, tgt}$}
    %\State{$MaskedST_{vct} \gets \Call{WaveSearch}{vct}$}
	\State{$MaskedST[vct] \gets \Call{WaveSearch}{vct}$}
    %\State{$RI_{ij,cand}[tgt] \gets \text{SET\_DIFF}(ST[vct], MaskedST[vct])$}
    \State{$RI_{ij,cand}[tgt] \gets \text{DIFF}(ST[vct], MaskedST[vct])$}
    %\State{$\Call{WaveUnlock}{aggr}$}
\EndFor

\State{$\Call{WaveUnlock}{aggr}$}

\State{$RI_{ij,or} \gets$ OR $RI_{ij,cand}$} \Comment{Determine the relation index}
\State{$RI_{ij} \gets$ $RI_{ij,cand} * flip$}
\State{\textbf{return} $RI_{ij}$}


% TODO: Maybe don't need to mention about error handling
%\If{$r_{ij,0} = r_{ij,1}$}\Comment{Determine the relation index}
%    \State{$r_{ij} \gets r_{ij,0}$ \textbf{OR} $r_{ij,1}$}
%    \Return{$r_{ij}$}
%\Else
%    \Return ERROR
%\EndIf

\end{algorithmic}
\end{algorithm}



%\begin{algorithm}
%\caption{Relation Search}
%\label{alg:rs}
%\begin{algorithmic}[1]
%%\INPUT{\ \\
%%Current microring index $i$\\
%%Next microring index $j$\\
%%Current microring search table $ST$
%%}
%\INPUT{Microring index pair $i$,$j$ and search table $ST$}
%\OUTPUT{Relation index $r_{ij}$}
%
%\State{Initialize $r_{ij,cand}[2]$ and $MaskedST_{vct}$}
%
%\If{$i \leq j$}\Comment{Determine aggressor/victim}
%    \State{$aggr, vct, flip \gets i, j, 1$}
%\Else
%    \State{$aggr, vct, flip \gets j, i, -1$}
%\EndIf
%
%%\State{/* Find the relation by microring aggression, Fig.X /*}
%
%\For{$tgt \gets 0, -1$}\Comment{Fig.X (a),(b), respectively}
%    \State{$\Call{WaveLock}{aggr, tgt}$}
%    \State{$MaskedST_{vct} \gets$ \Call{WaveSearch}{vct}}
%    \State{$r_{ij,cand}[tgt] \gets$ SET\_DIFF$(ST[vct], MaskedST_{vct})$}
%    \State{$\Call{WaveUnlock}{aggr}$}
%\EndFor
%
%\State{$r_{ij,or} \gets$ OR $r_{ij,cand}$} \Comment{Determine the relation index}
%\State{\textbf{return} $r_{ij,or} * flip$}
%
%
%% TODO: Maybe don't need to mention about error handling
%%\If{$r_{ij,0} = r_{ij,1}$}\Comment{Determine the relation index}
%%    \State{$r_{ij} \gets r_{ij,0}$ \textbf{OR} $r_{ij,1}$}
%%    \Return{$r_{ij}$}
%%\Else
%%    \Return ERROR
%%\EndIf
%
%\end{algorithmic}
%\end{algorithm}



%\begin{algorithm}
%%\label{alg:relation_search}
%\caption{Relation Search}
%\begin{algorithmic}[1]
%%\INPUT{\ \\
%%Current microring index $i$\\
%%Next microring index $j$\\
%%Current microring search table $ST$
%%}
%\INPUT{Microring index pair $i$,$j$ and search table $ST$}
%\OUTPUT{Relation index $r_{ij}$}
%
%\State{Initialize $MaskedST_{vct}$}
%
%\If{$i \leq j$}\Comment{Determine aggressor/victim}
%    \State{$aggr, vct, flip \gets i, j, 1$}
%\Else
%    \State{$aggr, vct, flip \gets j, i, -1$}
%\EndIf
%
%%\State{/* Find the relation by microring aggression, Fig.X /*}
%
%\State{$\Call{WaveLock}{aggr, 0}$}\Comment{Fig.X (a)}
%\State{$MaskedST_{vct}\gets$ \Call{WaveSearch}{vct}}
%\State{$r_{ij,0} \gets$ \textbf{SET\_DIFF}$(ST[vct], MaskedST_{vct})$}
%\State{$\Call{WaveUnlock}{aggr}$}
%
%\State{$\Call{WaveLock}{aggr, -1}$}\Comment{Fig.X (b)}
%\State{$MaskedST_{vct}\gets$ \Call{WaveSearch}{vct}}
%\State{$r_{ij,1} \gets$ \textbf{SET\_DIFF}$(ST[vct], MaskedST_{vct})$}
%\State{$\Call{WaveUnlock}{aggr}$}
%
%%\Return{$r_{ij,0} \textbf{OR} r_{ij,1}$}
%\State{$r_{ij,or} \gets r_{ij,0}$ \textbf{OR} $r_{ij,1}$} \Comment{Determine the relation index}
%\Return{$r_{ij,or} * flip$}
%
%% TODO: Maybe don't need to mention about error handling
%%\If{$r_{ij,0} = r_{ij,1}$}\Comment{Determine the relation index}
%%    \State{$r_{ij} \gets r_{ij,0}$ \textbf{OR} $r_{ij,1}$}
%%    \Return{$r_{ij}$}
%%\Else
%%    \Return ERROR
%%\EndIf
%
%\end{algorithmic}
%\end{algorithm}




==> include/alg_vtrs.tex <==


\begin{algorithm}
\caption{Variation-Tolerant Relation Search}
\label{alg:vtrs}
\begin{algorithmic}[1]
%\INPUT{\ \\
%Current microring index $i$\\
%Next microring index $j$\\
%Current microring search table $ST$
%}
\INPUT{Microring index pair $i$,$j$ and search table $ST$}
\OUTPUT{Relation index $r_{ij}$}

\State{Initialize $r_{ij,cand}[3]$ and $MaskedST_{vct}$}

\If{$i \leq j$}\Comment{Determine aggressor/victim}
	\State{$aggr, vct, flip \gets i, j, 1$}
\Else
	\State{$aggr, vct, flip \gets j, i, -1$}
\EndIf

%\State{/* Find the relation by microring aggression, Fig.X /*}

%\State{// Added tgt=1 from Alg.1 for Fig.X (c) and (d)}
%\For{$aggr\_tgt \gets 0, -1, 1$}\Comment{Fig.X (a,b) and (c,d)}
\For{$tgt \gets 0, -1, 1$}\Comment{Fig.X (a),(b) and (c,d)}
	%\State{$\Call{WaveLock}{aggr, aggr\_tgt}$}
	\State{$\Call{WaveLock}{aggr, tgt}$}
	\State{$MaskedST_{vct} \gets$ \Call{WaveSearch}{vct}}
	%\State{$r_{ij,cand}[aggr\_tgt] \gets$ \textbf{SET\_DIFF}$(ST, Masked ST)$}
	\State{$r_{ij,cand}[tgt] \gets$ SET\_DIFF$(ST[vct], MaskedST_{vct})$}
	\State{$\Call{WaveUnlock}{aggr}$}
\EndFor

\State{$r_{ij,or} \gets$ OR $r_{ij,cand}$} \Comment{Determine the relation index}
\State{\textbf{return} $r_{ij,or} * flip$}

% TODO: Maybe don't need to mention about error handling
%\If{$r_{ij,0} = r_{ij,1}$}\Comment{Determine the relation index}
%    \State{$r_{ij} \gets r_{ij,0}$ \textbf{OR} $r_{ij,1}$}
%    \Return{$r_{ij}$}
%\Else
%    \Return ERROR
%\EndIf

\end{algorithmic}
\end{algorithm}




==> include/archive/tab_model_params.tex <==


% Disclamer: Using booktabs package
% Reference - https://people.inf.ethz.ch/markusp/teaching/guides/guide-tables.pdf
% Summary of model parameters

\begin{table}[!t]

%\caption{Summary of Model Parameters\label{tab:model_params}}
\caption{Summary of Model Parameters}
\label{tab:model_params}
\ra{1.3}
\centering

\begin{tabular}{@{}lllp{40mm}@{}}
\toprule
\phantom{abc} & Symbol & Value & Description\\ \midrule
%\multicolumn{4}{@{}l}{WDM Grid}\\
DWDM Grid \\
 & $N_{ch}$ & 8 & Number of DWDM channels\\
 & $\lambda_{gS}$ & 1.12nm & Grid spacing\\
 & $\sigma_{gO}$ & 15nm & Grid offset between microring row and laser grid\\
 %& $\lambda_{gB}$ & 4.48nm & Fabrication bias\\
 %& $\{s_{i}\}$ & Nat./Perm. & (Target) spectral ordering\\ \midrule
 & $\{s_{i}\}$ & Nat. & Final microring spectral ordering at post-arbitration\\ \midrule
MWL Laser \\
 & $\sigma_{lGV}$ & $-$ & Global wavelength variation\\
 & & & (Accounted in $\sigma_{gO}$)\\
 %& $\sigma_{lLV}$ & 0.28nm & Local wavelength variation\\ \midrule
 & $\sigma_{lLV}$ & 25\% & Local wavelength variation\\ \midrule
Microring Row \\
 %& $\{\lambda_{i}\}$ & Nat./Perm. & Physical ordering in a row\\
 %& $\{r_{i}\}$ & Nat./Perm. & Physical ordering in a row\\ % Essentially a ring radius increment ordering
 %& $\{r_{i}\}$ & Nat. & Physical ordering in a row\\ % Essentially a ring radius increment ordering
 & $\{r_{i}\}$ & Nat. & Physical ordering in a row by ring radius increment\\ % Essentially a ring radius increment ordering
 & $\lambda_{rB}$ & 4.48nm & Fabrication bias\\
 %& & & Nat. = [0,1,2,3,4,5,6,7]\\
 %& & & Perm. = [0,4,1,5,2,6,3,7]\\
 & $\sigma_{rGV}$ & $-$ & Global resonance variation\\
 & & & (Accounted in $\sigma_{gO}$)\\
 & $\sigma_{rLV}$ & 2.24nm & Local resonance variation\\
 & $\lambda_{rFM}$ & 8.96nm & Mean FSR\\
 & $\sigma_{rFV}$ & 1\% & FSR variation\\
 & $\lambda_{rTM}$ & 1nm & Mean tuning range\\
 & $\sigma_{rTV}$ & 10\% & Tuning range variation\\
\bottomrule
%\multicolumn{4}{@{}l}{\footnotesize * $\sigma_{*}$ parameters model confidence interval bounds, i.e., [-$\sigma_{*}$, +$\sigma_{*}$]}\\
\multicolumn{4}{@{}l}{\footnotesize * $\sigma_{*}$ models confidence interval bound of variations, i.e., [-$\sigma_{*}$, +$\sigma_{*}$]}\\
\multicolumn{4}{@{}l}{\footnotesize ** Assuming O-band, 0.56nm is equivalent to 100GHz }\\
\multicolumn{4}{@{}l}{\footnotesize *** Nat.\ stands for natural ordering i.e., [0,1,2,3,4,5,6,7]}\\
%\multicolumn{4}{@{}l}{\footnotesize *** Nat.\ stands for natural ordering i.e., [0,1,2,3,4,5,6,7] whereas}\\
%\multicolumn{4}{@{}l}{\footnotesize \hspace{5mm}Perm.\ stands for permuted ordering i.e., [0,4,1,5,2,6,3,7]}\\
\end{tabular}
\end{table}



==> include/tab_alg_notation.tex <==


\begin{table}[h]

%\caption{Simulation Parameters\label{tab:sim_params}}
%\caption{Arbiter Configurations}
\caption{Lock-to-Cyclic Algorithm Denotation in \mysecref{scheme-eval}}
\label{tab:alg_notation}
\ra{1.3}
\centering

%\begin{tabular}{@{}lllp{35mm}@{}}
\begin{tabular}{@{}llll@{}}
%\begin{tabular}{@{}p{20mm}llll@{}}
\toprule
 \textbf{Algorithm} & RS/STM & VT-RS/STM & Seq. Tuning\\ 
\midrule
 %\multicolumn{4}{@{}l}{WDM Grid}\\
 %Target Policy & \multicolumn{3}{c}{Lock-to-Cyclic} \\
 %Pre-fab. Order$^1$ & Natural$^1$ & Permuted$^2$ & Natural & Permuted\\
 Record (\mysecref{scheme-record}) & Relation Search & Variation-Tolerant & -\\
 Matching (\mysecref{scheme-match}) & Single-Step Matching & Single-Step Matching & Lock-to-Nearest \\
 %$\left(s_i\right)^2$ & \multicolumn{2}{c}{Any} & Natural & Permuted\\
 %$\left(r_i\right)$ & Natural$^1$ & Permuted$^2$ & Natural & Permuted\\
 %$\left(r_i\right)$ & Natural$^1$ & Natural & Permuted$^2$ & Permuted\\
 %$\left(r_i\right)$ & Natural & Natural & Permuted & Permuted\\
 %$\left(s_i\right)$ & Any & Any & Natural & Permuted\\
\bottomrule
%\multicolumn{4}{@{}l}{\footnotesize * $\sigma_{*}$ parameters model confidence interval bounds, i.e., [-$\sigma_{*}$, +$\sigma_{*}$]}\\
%\multicolumn{4}{@{}l}{\footnotesize ** Assuming O-band, 0.56nm is equivalent to 100GHz }\\
%\multicolumn{4}{@{}l}{\footnotesize *** Nat.\ stands for natural ordering i.e., [0,1,2,3,4,5,6,7] whereas}\\
%\multicolumn{4}{@{}l}{\footnotesize \hspace{5mm}Perm.\ stands for permuted ordering i.e., [0,4,1,5,2,6,3,7]}\\

\end{tabular}
\end{table}



==> include/tab_sim_params.tex <==


% Disclamer: Using booktabs package
% Reference - https://people.inf.ethz.ch/markusp/teaching/guides/guide-tables.pdf
% Summary of model parameters

\begin{table}[!t]

%\caption{Simulation Parameters\label{tab:sim_params}}
\caption{Simulation Parameters}
\label{tab:sim_params}
\ra{1.3}
\centering

\begin{tabular}{@{}llp{50mm}@{}}
\toprule
Symbol & Value & Description\\ \midrule
%\multicolumn{4}{@{}l}{WDM Grid}\\
 $N_{\text{ring}}$ & 100 & Number of microring row samples\\
 $N_{\text{laser}}$ & 100 & Number of multi-wavelength laser samples\\
 %$P_{\sigma_*}$ & Uniform & Sample distribution of variations\\
 %$\sigma_{gO}$ & 15nm & Grid offset between microring row and laser grid\\
 %$\lambda_{gB}$ & 4.48nm & Fabrication bias\\
 %$\{s_{i}\}$ & Nat./Perm. & (Target) spectral ordering\\ \midrule
\bottomrule
%\multicolumn{4}{@{}l}{\footnotesize * $\sigma_{*}$ parameters model confidence interval bounds, i.e., [-$\sigma_{*}$, +$\sigma_{*}$]}\\
%\multicolumn{4}{@{}l}{\footnotesize ** Assuming O-band, 0.56nm is equivalent to 100GHz }\\
%\multicolumn{4}{@{}l}{\footnotesize *** Nat.\ stands for natural ordering i.e., [0,1,2,3,4,5,6,7] whereas}\\
%\multicolumn{4}{@{}l}{\footnotesize \hspace{5mm}Perm.\ stands for permuted ordering i.e., [0,4,1,5,2,6,3,7]}\\
\end{tabular}
\end{table}


